User Pairing and Power Allocation for IRS-Assisted NOMA Systems with Imperfect Phase Compensation

In this letter, we analyze the performance of the intelligent reflecting surface (IRS) assisted downlink non-orthogonal multiple access (NOMA) systems in the presence of imperfect phase compensation. We derive an upper bound on the imperfect phase compensation to achieve minimum required data rates for each user. Using this bound, we propose an adaptive user pairing algorithm to maximize the network throughput. We then derive bounds on the power allocation factors and propose power allocation algorithms for the paired users to achieve the maximum sum rate or ensure fairness. Through extensive simulations, we show that the proposed algorithms significantly outperform the state-of-the-art algorithms.

==> Appendices.tex <==
\appendices
\section{Proof of Lemma 1}
\label{sec:Lemma1}
%\begin{proof}
We adopt the \gls{SINR} approximation formulated in~\cite{MISO} and define the following:
\begin{align}
    \Bigg|\dfrac{1}{N}\sum_{n=1}^{\gls{N}} e^{j\gls{thetak'}}\Bigg|^2 \overset{\text{\scriptsize(a)}}{\longrightarrow} \big|\mathbb{E}[e^{j\gls{thetak'}}]\big|^2\overset{\text{\scriptsize (b)}}{=} \big|\mathbb{E}[\cos(\gls{thetak'})]\big|^2\overset{\text{\scriptsize (c)}}{=}\sinc^2(\gls{delta}),
\label{eqn:sinc2}
\end{align}
where $(a)$ is based on law of large numbers~\cite{MISO}, $(b)$ is obtained by integrating the odd symmetrical function  $\sin(\gls{thetak'})$ for $\gls{thetak'}\in[-\gls{delta}, \gls{delta}]$, and $(c)$ uses the probability density function of \gls{thetak'} which is defined as $f(\gls{thetak'})=\frac{1}{2\gls{delta}}, \forall \gls{thetak'}\in[-\gls{delta},\gls{delta}]$ and ${\sinc (\gls{delta})=\frac{\sin (\gls{delta})}{\gls{delta}}}$. Substituting \eqref{eqn:c1}-\eqref{eqn:GammaCSI} and \eqref{eqn:sinc2} in \eqref{eqn:GammaO}-\eqref{eqn:Gamma2N}, we get
\begin{align}
\gls{GammaIO}=&\dfrac{\gls{Pt}|\gls{PLi}\gls{PLI}|^2\big|\sum_{n=1}^{\gls{N}} e^{j\gls{thetak'}}\big|^2 M}{\gls{I}+\gls{sigma2}}=\gls{GammaCSI}\sinc^2(\gls{delta}), \forall i=1,2,\label{eqn:GammaOU}\\
\gls{GammaS}=&\dfrac{\gls{a1}\gls{Pt}|\gls{PL1}\gls{PLI}|^2\big|\sum_{n=1}^{\gls{N}} e^{j\gls{thetak'}}\big|^2 M}{\gls{I}+\gls{sigma2}}=\gls{a1}\gls{Gamma1CSI}\sinc^2(\gls{delta}),\label{eqn:Gamma2NU}\\
\gls{GammaW}=&\dfrac{\gls{a2}\gls{Pt}|\gls{PL2}\gls{PLI}|^2\big|\sum_{n=1}^{\gls{N}} e^{j\gls{thetak'}}\big|^2 M}{\gls{a1}\gls{Pt}|\gls{PL2}\gls{PLI}|^2\big|\sum_{n=1}^{\gls{N}} e^{j\gls{thetak'}}\big|^2 M+\gls{I}+\gls{sigma2}},\nonumber\\
=&\dfrac{\gls{a2}\gls{Gamma2CSI}\sinc^2(\gls{delta})}{\gls{a1}\gls{Gamma2CSI}\sinc^2(\gls{delta})+1}.
\label{eqn:Gamma2NU}
\end{align}
Assuming the full bandwidth allocation for the two users in case of \gls{NOMA} and half bandwidth allocation for each user in \gls{OMA}, and substituting \eqref{eqn:GammaOU}-\eqref{eqn:Gamma2NU} while calculating the normalized data rates, we complete the proof. \hspace{2.8cm} \qedsymbol %\end{proof}
